Numerical Analysis of Diagonal-Preserving, Ripple-Minimizing and Low-Pass Image Resampling Methods

Image resampling is a necessary component of any operation that changes the size of an image or its geometry. Methods tuned for natural image upsampling (roughly speaking, image enlargement) are analyzed and developed with a focus on their ability to preserve diagonal features and suppress overshoots. Monotone, locally bounded and almost monotone "direct" interpolation and filtering methods, as well as face split and vertex split surface subdivision methods, alone or in combination, are studied. Key properties are established by way of proofs and counterexamples as well as numerical experiments involving 1D curve and 2D diagonal data resampling. In addition, the Remez minimax method for the computation of low-cost polynomial approximations of low-pass filter kernels tuned for natural image downsampling (roughly speaking, image reduction) is refactored for relative error minimization in the presence of roots in the interior of the interval of approximation and so that even and odd functions are approximated with like polynomials. The accuracy and frequency response of the approximations are tabulated and plotted against the original, establishing their rapid convergence.

==> LiteratureReview.tex <==
\chapter{Literature Review: FIR Filter Design with Chebyshev and
  Minimax Methods}
\label{chap:Literature}

This chapter presents a brief review of the literature concerning FIR
(Finite Impulse Response) \nomenclature{FIR}{Finite Impulse
  Response}\index{FIR Filter Design} filter design using Chebyshev and
minimax method\index{Chebyshev FIR Filter Design}\index{Minimax FIR Filter Design}.  A survey of some of the important methods and
improvements are presented, along with a brief description.

\section{Background}

A Finite Impulse Response (FIR)\index{FIR Filter} filter is a digital filter whose values become null after a finite amount of time.  The impulse response\index{Impulse Response} of a filter is the result of applying a signal consisting of a single maximal non-zero value.  By contrast, Infinite Impulse Response (IIR) filters\index{IIR Filter} \nomenclature{IIR}{Infinite Impulse Response} are digital filters whose values stretch out to infinity.  In this chapter, the focus will be on FIR filter design\index{FIR Filter Design} methods.  The frequency response\index{Frequency Response} of an FIR digital filter is a function, usually complex, of the frequency after normalization \citep{ChenParks}.

There are many reasons for designing FIR filters\index{FIR Filter}.  They have many applications in signal processing, including image processing, geophysical data processing, radar data processing \citep{Charalambous}, nearly linear-phase filtering, and equalization \citep{BurnsideParks}.  They are very attractive for such applications because of certain properties they possess \citep{Rabiner}.  For instance, they can have exactly linear phase\index{Exactly Linear Phase}, they do not pose the same stability problems as IIR filters\index{IIR Filter}, and they can be quite easy to design \citep{Charalambous}, due to the many efficient methods available \citep{McClellanParks}.  In fact, during the 70's and 80's, many researchers have given some thought to the problem of designing optimum (in the Chebyshev sense) FIR filters\index{Chebyshev FIR Filter Design} \citep{MianNainer, Charalambous}, both in the one-dimensional and two-dimensional cases.  Most of this research has been focused on the design of linear-phase FIR filters\index{Linear-Phase FIR Filter} \citep{MianNainer}, since this can be an important characteristic \citep{Charalambous}, though it not always required and may be unwanted \citep{MianNainer}. 

Many different solutions to the classical problem of FIR filter
design\index{FIR Filter Design} in one or more dimensions have been
proposed \citep{Algazi}.  Some very powerful and computationally
efficient algorithms have been developed, particularly for the
linear-phase case\index{Linear-Phase FIR Filter} \citep{MianNainer}.
When there are constraints in the time domain, linear
programming\index{Linear Programming} is one of the popular techniques
for FIR filter design\index{FIR Filter Design}
\citep{Samueli}. 
Other techniques have also been considered for the various cases.
Researchers have also been interested in the design of filters with
certain behaviours in two or more bands \citep{Preuss}.

An example where filters with constraints in the time domain are useful is in the sections of data communication systems responsible for transmitting and receiving.  The transmit filter must constrain the spectrum of the transmitted data so it fits into bandlimited channels while the receive filter must reject the noise that is outside of the band and maximize the signal-to-noise ratio \citep{Samueli}.  In this case, there are constraints in the time domain since the impulse response\index{Impulse Response} of the transmit and receive filters have zero-crossings at uniform distances from one another; such filters are known as Nyquist filters\index{Nyquist Filter} \citep{Samueli}.

\section{Statement of the Problem}
\index{FIR Filter Design!Problem Statement}

The design and realization of a digital filter can be separated into five steps \citep{Rabiner}.  The first step consists of choosing the technique that will be used for the design of the filter and writing the desired filter specifications mathematically.  The next step is a key step where the ideal filter is approximated by solving the problem to find the coefficients which minimize an error function.  The third step consists of choosing the structure to realize the filter and then quantizing the filter coefficients so that they have a fixed length.  The fourth step is quantizing the lengths of the filter variables and the fifth step is the verification that the resulting filter really does meet the desired specifications \citep{Rabiner}.  The literature that will be reviewed here will focus on the second step, which consists in solving the approximation problem.

The basic idea of the problem under consideration is finding an approximation of an ideal frequency response \citep{McClellanParks, Harris}.  Usually its magnitude is approximated, but the phase can also be considered \citep{Preuss}.  There are various minimization criterion which can be used, the most common being the Chebyshev error criterion\index{Chebyshev Error Criterion} and the weighted least squares (WLS) \nomenclature{WLS}{Weighted Least Squares} error criterion\index{WLS Error Criterion}.  Basically, the frequency response\index{Frequency Response} of an ideal filter\index{Ideal Filter} is known and the idea is to obtain an optimal approximation\index{Optimal Approximation} of this frequency response such that the error function is minimized \citep{Lim, BurnsideParks}, which can then be converted back into the time domain to obtain a digital filter.  This approximation can be done in one dimension, where it is generally easy, or in two dimensions, where the functions are generally complex and the problem become more computationally intensive.

In the two-dimensional case, the problem can be reformulated in the case where the filter is exactly linear phase\index{Exactly Linear Phase}, that is, when it has symmetric real coefficients.  In this case, one can use the Chebyshev error criterion\index{Chebyshev Error Criterion} and solve the problem as a real approximation problem \citep{ChenParks, Algazi}.  The approximating function can then be written as a weighted sum of cosine functions \citep{McClellanParks}.  

If, however, the filter to be approximated is not linear-phase, then the approximation problem becomes complex \citep{ChenParks}.  These problems tend to be more computationally intensive but there may also be advantages to solving the complex approximation problem.  One of its most important features is that by minimizing the error function, both the weighted magnitude error and the phase error are reduced simultaneously \citep{Preuss}.  However, the complex approximation problem can also be seen as a real approximation problem that is nonlinear, if that is preferred, since the norm of the error function can be rewritten as the usual norm of a complex number, that is, the square root of the sum of the squares of the real and imaginary parts of the error function \citep{BurnsideParks}.

The Chebyshev (or minimax) error criterion\index{Chebyshev Error Criterion}\index{Minimax Error Criterion} is often used because it corresponds to minimizing the extremal error over all frequencies \citep{Lim}.  Minimizing the Chebyshev norm leads the error function to have an equiripple behaviour\index{Equiripple}, where all the extrema of the error function have the same value \citep{Preuss}.  This is a well-known fact.  On the other hand, the weighted least squares (WLS)\index{WLS Filter Design} design method minimizes the weighted integral of the squared error function \citep{Algazi, Lim}.

Therefore, the approximation step of FIR filter design\index{FIR Filter Design} basically consists of finding the values of the coefficients of the impulse response\index{Impulse Response} such that the Chebyshev norm of the error\index{Chebyshev Error}, or the weighted least squares error\index{WLS Error}, is minimized, where the error function is defined as the weighted difference between the ideal filter which is being approximated and the resulting approximating function. \citep{Harris, ChenParks, Preuss}.

\section{History}


There have been many attempts at solving the FIR filter design\index{FIR Filter Design} problem.  Many researchers have considered solutions to the problem and tried to improve on the previously-developed methods.  Such improvements included convergence speed, computational complexity, numerical stability, and maximal filter size.  Here, a brief look will be taken at some of the major developments in solving the FIR filter design problem.  

One of the first methods used to solve the approximation problem was the method of windowing\index{Windowing} \citep{Rabiner}.  In its earlier stages, this consisted simply in taking the Fourier series\index{Fourier Series} of the ideal frequency response\index{Ideal Frequency Response} and truncating it to the required length.  An advantage of this method was that the least squares error was minimized but a disadvantage was that the Chebyshev error\index{Chebyshev Error} was not.  In fact, the Gibbs phenomenon\index{Gibbs Phenomenon} could cause this error to be quite large \citep{Rabiner}. 

Later on, the technique of windowing was refined such that the Fourier series\index{Fourier Series} was not simply truncated.  Rather, its coefficients were multiplied by a time-limited window\index{Time-Limited Window}.  This method was developed to reduce the Gibbs phenomenon\index{Gibbs Phenomenon} that had previously caused the Chebyshev error to be large \citep{Rabiner}.  Many windows were developed and used.  Some of the more popular ones included the Kaiser\index{Kaiser Window} \citep{Kaiser}, the Hamming\index{Hamming Window} \citep{Blackman}, and the Dolph-Chebyshev\index{Dolph-Chebyshev Window} \citep{Dolph} windows.  An advantage of this method was that the windowing\index{Windowing} technique was analytical rather than iterative like most of the other methods for FIR filter design\index{FIR Filter Design} \citep{Rabiner}.

In 1961, Lawson \citep{Lawson} described a new iterative method to solve this approximation problem.  This algorithm became fundamental for finding optimal approximations\index{Optimal Approximation}\index{Polynomial of Best Approximation} in the Chebyshev sense \citep{ChenParks}.  This algorithm works on the idea that the best approximation in the Chebyshev sense is a weighted $L_p$ approximation, where the weighting is unknown \citep{BurnsideParks}.  This algorithm recursively finds this weighting function as well as the extremal set \citep{ChenParks} and eventually converges to the optimal approximation in the Chebyshev sense \citep{BurnsideParks}.  However, the algorithm seems to have a slow convergence rate \citep{ChenParks} and, worse, it often stops before reaching the optimal solution.  This seems to happen when the weighting function becomes zero at certain points.  Methods have been proposed to deal with this problem and they typically get the algorithm to restart \citep{BurnsideParks}.  Due to this need to restart the algorithm, the convergence of the method is more difficult to show \citep{BurnsideParks}.

A few years later, the frequency sampling method\index{Frequency Sampling Method} was published by Gold and Jordan \citep{GoldJordan}.  This technique has been applied to a variety of problems, including band-pass\index{Band-pass Filter} and low-pass filters\index{Low-Pass Filter} \citep{McClellanParks}.  Basically, this method works by fixing values for the coefficients of the discrete Fourier transform\index{Discrete Fourier Transform} everywhere except in the transition bands.  These values are then optimized using an algorithm that minimizes a weighted approximation error \citep{Rabiner}.  However, disadvantages with this method are that the result is not optimal in the Chebyshev sense, and it is also not possible to specify the frequencies at the edge of the bands \citep{McClellanParks}.  This is a linear programming\index{Linear Programming} problem where there are few variables but many constraints \citep{Rabiner}.  This method was improved upon by Rabiner et al. \citep{RabinerGold}.

In 1970, Herrmann \citep{Herrmann} developed the first method for the design of optimal FIR filters\index{Optimal Approximation}\index{FIR Filter} in the Chebyshev sense \citep{Rabiner}.  His method was based on the assumption that there was an equiripple property\index{Equiripple} of the optimal low-pass filter\index{Low-Pass Filter} in each band.  Then, he simply fixed the amount of ripples in the bands and this led to some nonlinear equations, which could then be solved.  In this case, Herrmann used an iterative descent method\index{Iterative Descent Method} \citep{Rabiner}.  At the same time, Herrmann and Schuessler \citep{HerrmannSchuessler} described a way for going from equiripple linear-phase designs\index{Equiripple Linear-Phase Design} to equiripple minimum-phase designs\index{Equiripple Minimum-Phase Design}.  This way, they ended up with half the original degree \citep{MianNainer}.  Filters developed using Herrmann's method had the disadvantage of being rather small.  Their size was limited to $40$ \citep{Rabiner}.

The next year, Herrmann's method was improved upon by Hofstetter et al. \citep{Hofstetter}, who made it possible to design longer filters.  They developed another algorithm for solving the nonlinear equations, instead of using the iterative descent method like Herrmann.  Their new algorithm was similar to the Remez exchange algorithm\index{Remez Algorithm} \citep{Rabiner}.  The resulting filters were optimum\index{Optimal Approximation} in the Chebyshev sense but belonged to a restricted class of such filters \citep{McClellanParks}.  These were called extraripple filters\index{Extraripple Filter}, or maximal ripple filters\index{Maximal Ripple Filter}.  Extraripple filters have only one more ripple than the minimum need for optimality \citep{Rabiner}.  One disadvantage of this method, as well as of Herrmann's method is that the cutoff frequencies of the bands cannot be specified beforehand \citep{Rabiner}.

Regarding the design of linear phase\index{Linear Phase Filter} FIR filters\index{FIR Filter} in two dimensions, one of the simplest algorithms was a windowing\index{Windowing} method published by Huang in 1972 \citep{Huang}.  However, this method was not optimal in any sense \citep{Charalambous}.

The same year, Parks and McClellan \citep{ParksMcClellan72} showed that the Remez algorithm\index{Remez Algorithm} \citep{Remez1} was a good method for computing best approximations in the Chebyshev sense \citep{McClellanParks, Rabiner}.  They approximated an ideal frequency response\index{Ideal Frequency Response} for a low-pass filter\index{Low-Pass Filter} in the pass-band and the stop-band using the Remez exchange algorithm\index{Remez Algorithm}\citep{Rabiner}.  This method has been used to design linear phase FIR filters\index{FIR Filter}\index{Linear Phase Filter}.

Around the same time, Rabiner \citep{Rabiner72} proposed an alternative to the method using the Remez exchange algorithm.  He demonstrated that linear programming\index{Linear Programming} could also be used to obtain optimal approximations\index{Optimal Approximation} in the Chebyshev sense \citep{Rabiner}.  In fact, one can design the same filter using both the Remez algorithm\index{Remez Algorithm} and linear programming\index{Linear Programming} \citep{McClellanParks}.  There is a difference between the two, however.  An advantage of linear programming is that it is flexible and can be used to design filters of various shapes \citep{Rabiner}.  On the other hand, the Remez algorithm requires much less time to perform, and thus can design longer filters \citep{McClellanParks}.

Hu and Rabiner \citep{HuRabiner} then proposed a method whereby linear programming\index{Linear Programming} is directly applied to the FIR filter design\index{FIR Filter Design} problem.  This method consists of applying linear programming in a straightforward manner \citep{Harris, Charalambous}.  It has been deemed a slow method \citep{Charalambous} but can design a filter for a small circularly symmetric impulse response in about an hour \citep{Harris}.

In 1973, McClellan \citep{McClellan73} proposed another method for the design of equiripple linear-phase FIR filters\index{Equiripple}\index{Linear-Phase FIR Filter}\index{FIR Filter}.  This is a relatively simple method for designing two-dimensional filters.  An appropriate polynomial mapping is applied to a one-dimensional ideal filter to then obtain a two-dimensional filter \citep{Harris}.  The result is equiripple but it is not always optimal in the Chebyshev or minimax sense \citep{Charalambous}.  Another disadvantage is that the magnitude function must be carefully chosen since they cannot all be approximated well \citep{Harris}.  However, there are advantages to this method.  It is easy to use to design FIR filters and the results usually have efficient implementations \citep{Harris}.

The same year, Fisher \citep{Fisher} proposed using the Lawson algorithm\index{Lawson Algorithm} \citep{Lawson} for approximations in the complex frequency domain\index{Complex Frequency Domain}.  However, this method seems to not have worked very well \citep{ChenParks}.

Then, Mueller \citep{Mueller} considered the design of FIR Nyquist digital filters\index{Nyquist Filter} using an eigenvalue problem.  He presented a numerical solution to this problem \citep{Samueli}.

Later, Burris \citep{Burris} worked on the method of Herrmann and Schuessler \citep{HerrmannSchuessler} and decided to generalize it.  His method consisted of solving for the roots of a polynomial and factoring these roots in a suitable manner to get the minimum-phase counterpart \citep{MianNainer}.

Fiasconaro \citep{Fiasconaro} studied the method proposed by Hu and Rabiner \citep{HuRabiner} and wanted to improve on the amount of time required to solve the approximation problem.  He decided to propose an adaptive algorithm in which the solution from each iteration was optimized using linear programming\index{Linear Programming}.  However, this method still required a fair amount of time \citep{Harris}.

The descent algorithm\index{Descent Algorithm} was applied to the FIR
filter design problem by Kamp and Thiran \citep{KampThiran} and by
Hersey and Mersereau \citep{HerseyMersereau} in an independent
fashion.  They managed to improve on the time required for the
solution of the approximation problem, but the filter footprint was
still limited to about $15\times15$ because of the computational
complexity of the method \citep{Harris}.  Harris \citep{Harris76} also
developed a similar ascent minimax algorithm\index{Minimax Algorithm}.
There were also numerical difficulties encountered in the
implementation of these algorithms \citep{Charalambous}.  These
difficulties were due to degeneracy in the reference functions
\citep{Charalambous}.

There were also researchers who described the approximation problem and some of the theory behind it.  Rivlin and Shapiro \citep{Rivlin74, RivlinShapiro} focused on a demonstration that the best least squares approximation using a good weighting function is the same as an optimal approximation in the Chebyshev sense \citep{ChenParks}.  At this point, if the weighting function is known along with the set of extrema, then the optimal complex minimax approximation\index{Optimal Approximation} can be found using least squares \citep{ChenParks}.

In 1978, Barrodale et al. \citep{Barrodale} suggested using a Taylor expansion\index{Taylor Expansion} to linearize the approximation problem and then using a previously-published algorithm to solve it.  However, the solution obtained can have a large error since the Taylor expansion is not accurate \citep{ChenParks}.  They then suggested the use of a perturbation method to get a better approximation.  This method was not very reliable and could fail even for small problems \citep{ChenParks}.

Instead of trying to approximate both the real and imaginary parts of FIR filters, Steiglitz \citep{Steiglitz} proposed separate approximations for these.  However, a disadvantage of this method is that the errors for the magnitude and for the phase are not adjustable \citep{ChenParks}.

Around the same time, Glashoff and Roleff \citep{GlashoffRoleff} and Streit and Nuttall \citep{StreitNuttall} independently suggested that the approximation problem be discretized and converted from the complex domain to the real domain.  Glashoff and Roleff solved the linear real problem and used that solution as an initial vector for the Newton-Raphson method\index{Newton-Raphson Method} \citep{ChenParks}.  However, it is not guaranteed that the Newton-Raphson iteration will converge if the initial guess is not a good one \citep{ChenParks}.  Streit and Nuttall had a set of overdetermined linear equations and used a linear programming\index{Linear Programming} algorithm directly to solve them \citep{ChenParks}.  They minimized the error only on a grid, and the grid density could be manipulated to reduce the error \citep{BurnsideParks}.  An advantage of their method was that their linear programming algorithm was stable and there was no need for an initial vector.  However, it did take a long time to compute large filters \citep{ChenParks}.

A few years later, Lim and Parker \citep{LimParker} showed that it is valid to used the weighted least squares method for designing large FIR filters when the coefficient space is discrete \citep{Lim}.

Later, Cortelazzo and Lightner \citep{CortelazzoLightner} published a method for designing FIR and IIR filters\index{FIR Filter}\index{IIR Filter} that could approximate either the magnitude, the phase, or the group delay of an ideal filter \citep{ChenParks}.  However, this method was time-consuming and only worked well when the FIR filter was no longer than ten \citep{ChenParks}.

In 1987, Saram\"{a}ki and Neuvo \citep{SaramakiNeuvo} developed an algorithm which used the Parks-McClellan method\index{Parks-McClellan Algorithm} to optimize in the frequency domain while at the same time optimizing in the time domain by solving linear equations \citep{Samueli}.  This is an iterative method to design equiripple FIR Nyquist filters\index{Equiripple}\index{Nyquist Filter}\index{FIR Filter} and may need some modifications depending on the application.  It seems to be well-behaved numerically and is a good alternative to linear programming \citep{Samueli}.

The same year, Chen and Parks \citep{ChenParks} presented a method similar to that of Streit and Nuttall.  Their method used finitization, which adds a certain amount of error to the final solution \citep{BurnsideParks}.  Another disadvantage is that the method can be slow and use a lot of memory space when the filter length grows \citep{BurnsideParks}.  However, it can give pretty accurate solutions when used to design filters of length up to $50$ \citep{BurnsideParks}.

Later, Tang \citep{Tang88} developed an iterative method which did not involve finitization.  The approximation problem was solved by simply using a simplex algorithm\index{Simplex Algorithm} for linear programming directly \citep{BurnsideParks}.  This method can be used to design FIR filters\index{FIR Filter} with arbitrarily small Chebyshev errors \citep{BurnsideParks}.

Preuss \citep{Preuss, Preuss87} then published an interpolating method which is also iterative.  An advantage of this method is that its convergence is fast when compared to linear programming methods \citep{BurnsideParks}.  However, it can be numerically unstable and it is not known whether it always converges to the optimal solution \citep{BurnsideParks}.

Preuss' method was improved upon by Schulist \citep{Schulist} in 1990.  He made the method faster and dealt with some of the numerical instability problems \citep{BurnsideParks}.  Schulist also showed that it is possible to add linear constraints to the problem when using linear programming\index{Linear Programming} methods but this has not been shown to be the case for interpolating methods \citep{BurnsideParks}.

Tang's simplex algorithm\index{Simplex Algorithm} was applied by Alkairy et al. \citep{Alkairy91, Alkairy93} to FIR filter design.  They used Tang's method for the starting and then solved the linear equations by taking the inverse of the matrix \citep{BurnsideParks}.  The memory requirements, convergence speed, as well as accuracy were all greatly improved by this method.  As such, longer filters could now be designed \citep{BurnsideParks}.

A method different from the previous ones was proposed by Potchinkov and Reemtsen \citep{PotchinkovReemtsen} in 1992.  They formulated the FIR filter design\index{FIR Filter Design} problem as a quadratic problem, thus not requiring any linearization \citep{BurnsideParks}.  It is a fact that quadratic programming\index{Quadratic Programming} is more computationally intense than linear programming, but since there is no need for linearization, it is possible that the method allows for faster convergence \citep{BurnsideParks}.  Potchinkov and Reemtsen have designed filters that had lengths of up to $300$.

Tseng \citep{Tseng} decided to reconsider Lawson's algorithm\index{Lawson Algorithm} for FIR filter design\index{FIR Filter Design} and improved on the implementation of the method as well as on its tendency to stop prematurely \citep{BurnsideParks}.

In 1993, Burnside and Parks \citep{BurnsideParks93} published a multiple exchange linear programming method\index{Multiple Exchange}\index{Linear Programming} based on the simplex algorithm\index{Simplex Algorithm}.  They improved the starting method and the step where the linear equations are solved by finding an inverse matrix \citep{BurnsideParks}.  Their method was also generalized so it can be used to design complex FIR filters.  It is numerically stable and relatively fast \citep{BurnsideParks}.


\section{Literature Review}

\subsection{FIR Digital Filter Design Techniques Using Weighted Chebyshev Approximation -- Rabiner et al.}

In their paper, Rabiner et al. \citep{Rabiner} discuss various optimal
methods for obtaining the solution of the FIR design approximation
problem.  In this case, optimality is in the Chebyshev sense.  They
start out by explaining that the alternation theorem is very powerful
since it gives necessary and sufficient conditions for the optimal
Chebyshev solution.  The Remez exchange algorithm is based on this
theorem and is an efficient method for solving the approximation
problem.  However, the alternation theorem is only valid when the
basis functions satisfy the Haar condition; that is, each subset of
$n$ vectors is linearly independent \cite{Cheney}.  Unfortunately, in
two dimensions, these basis functions no longer satisfy the Haar
condition.  As such, it is then impossible to find the optimal
solution based on the alternation theorem.

When the filter is required to have the maximum number of extremal frequencies, it is possible to get a unique optimal filter.  Such filters are called maximal ripple filters, or extraripple filters in the case of low-pass filters.  In order to obtain a maximal ripple filter, one first gets a set of nonlinear equations by requiring the error function to attain a certain error value at the same time as having a zero derivative.  These equations can be solved by iteration using optimization techniques.  However, the maximum error value is fixed and therefore is not minimized.  Also, the method does not give freedom to specify where the band edges will be, instead selecting where these will be.  Another iterative method was proposed for designing such filters, this one based on the idea of obtaining a polynomial with chosen values at the extrema.  This method starts with an initial guess of the location of these extrema and then obtains a polynomial using Lagrange interpolation.  Then, the extrema of this polynomial are found and another iteration begins.  This is reminiscent of the Remez multiple exchange algorithm.  The algorithm will converge independently of the initial estimate, but certain estimates may require more or less iterations than others.  As with the previous method, it is still not possible to specify the filter band edge frequencies beforehand.

Other techniques such as linear programming can also be used to solve this approximation problem.  Linear programming is much slower than the Remez algorithm, however, since it is basically a single exchange method, whereas the latter is a multiple exchange method.  On the other hand, when constraints are added to the time domain, the Remez algorithm is not useful anymore and linear programming becomes the method of choice.  When designing low-pass filters, for example, there are constraints in both the time and frequency domains at the same time.  In this case, linear programming works well.  Another example where the linear programming method surpasses the Remez algorithm is in the design of interpolation filters with some null coefficients.  In this case, the Haar condition is not satisfied and thus the alternation theorem cannot be applied.

Designing FIR filters in two dimensions is typically much more difficult than designing such filters in one dimension.  Some techniques have been extended from one to two dimensions but for most techniques this does not work very well.  The Remez algorithm has not been extended to two dimensions as of 1975 and there are no efficient methods for the design of two-dimensional optimal FIR filters.  The problems with extending the Remez algorithm to two dimensions are that first, the Haar condition is not satisfied in two dimensions and thus the alternation theorem cannot be applied, and secondly, that there is no way of ordering the extrema such that the error sign changes from point to point.  For now, linear programming seems to be the best method to use, but it is limited to low-order filters.

\subsection{A Unified Approach to the Design of Optimum FIR Linear-Phase Digital Filters -- McClellan and Parks}

In this article, McClellan and Parks \citep{McClellanParks} discuss a method for designing FIR linear-phase digital filters where each possible case is reduced to an appropriate form for using the Remez exchange algorithm.  Basically, they show that there are four possible cases and that each can be modified and then solved using the Remez algorithm.  Until this moment, only certain types of filters could be designed using the Remez algorithm, and all others had to use linear programming, which tends to be slower.

Once all cases can be reduced to the one case which is solvable using the Remez algorithm, it is possible to approximate band-pass filters, band-stop filters, Hilbert-transform filters, differentiator filters, and any arbitrary filter using this algorithm.  Now that the theory shows that all cases can be reduced to a simple one, a more compact method can be found to compute the optimal approximation.  They state that there is only a need for an algorithm which will approximate using cosine functions, since this is the case to which all others can be reduced.  They also provide a Fortran program which is based on this idea.  Such a program takes in an input, formulates this input into the wanted approximation problem, solves this problem with the Remez algorithm, and calculates the impulse response from these results.  This method can be used for the design of FIR linear-phase digital filters.

\subsection{A Comparison of Algorithms for Minimax Design of Two-Dimensional Linear Phase FIR Digital Filters -- Harris and Mersereau}

In this paper, Harris and Mersereau \citep{Harris} compare two iterative FIR linear-phase digital filter design techniques which both use multiple-exchange ascent algorithms, and present a new algorithm which reduces the amount of iterations required for such algorithms.  The first method was developed by Kamp and Thiran and the second by Hersey and Mersereau.  Both of these methods are faster than linear programming techniques.

They propose three reasons for the reexamination of the ascent algorithms.  The first reason is that ascent algorithms result in optimal filters in the Chebyshev sense.  The second reason is that filters with any magnitude specification can be approximated using this method since it is general.  The third reason is that the optimal results from the ascent algorithm can then be used as a basis for applying the McClellan method.

The new algorithm they present is more efficient than both the Kamp and Thiran, and the Hersery and Mersereau algorithms.  It uses the beginning of the Hersey-Mersereau method but also adds in some useful features of the other algorithm.  This method is to be used for two-dimensional linear phase FIR digital filters.

Harris and Mersereau then explain that the algorithms they will compare are all iterative and guaranteed to converge, and that it is thus important to know when to stop.  They present some theorems of approximation theory which basically tell how to recognize when the best approximation has been obtained.

The ascent algorithm is a well-known method used for finding approximations on discrete sets of points which are optimal in the Chebyshev sense.  The discrete sets are usually simply samples of the continuous function taken on a Cartesian grid.  This grid must be dense enough.  If there are transition bands in the filter, the samples must include points along the edges of such bands.  The basic idea of the ascent algorithm is to make a sequence of best approximations on sets of points, changing these points such that the norm of the error is monotonically increasing.  The solution with the maximum norm on sets of points will be the same as the solution with the minimum norm on the whole discrete set.  First, an initial set of points is chosen.  Then, a best approximation is calculated, the error function is evaluated at all the points, and the maximum norm is found.  If the point with maximum norm is already in the chosen set of points, the algorithm ends.  Otherwise, it is exchanged with another point and the next iteration begins with the new set of points.  This is also called the single-exchange ascent algorithm.  This algorithm, however, can be slow to converge since only one point is exchange at each iteration.  The search for the largest error takes the most time.  A suggestion is to replace more than one point at a time.

The method of Kamp and Thiran is designed to find local maxima of the error function in little time.  They suggest starting at one of the reference points and moving horizontally while looking for a local maximum.  Once the maximum is found, one can move vertically to find another local maximum.  This continues until a local maximum is found both horizontally and vertically at the same time.  The same thing is done for each reference point and the results are added to the set of reference points.  If this method fails, then the overall maximum error is found, as in the original ascent algorithm.  If a single point is found, it is exchanged as previously but if more than one local maximum is found, they replace the reference points with the greatest errors.  A best approximation is only computed once per iteration.

The method of Hersey and Mersereau is based on the first Remez algorithm.  In this method, they use a sparse grid of points which contains the reference points from the previous iteration.  At each iteration, they find local maxima and add them to the set while removing those that have a small error.  They then use the single-exchange algorithm to determine the best approximation on this grid of points.  This approximation is used to search for the local maxima of the error function over the whole set of points.  The local maxima are then added to the grid of points and the next iteration starts.  Originally, the search over the whole set of points was simply an exhaustive search but they later added a variation of the search part of the Kamp and Thiran algorithm, allowing the search to also include diagonals.

The new algorithm proposed in this paper is the method of steepest ascent.  It is like the Hersey-Mersereau algorithm, but the exchange section is modified such that the worst error points on the sparse grid are exchanged for points in the reference set of points.  This leads to more calculations and more complex method but it also converged faster since less exchanges have to be performed.  This is particularly useful for high-order filters.

\subsection{A Fast Procedure to Design Equiripple Minimum-Phase FIR Filters -- Mian and Nainer}

Here, Mian and Nainer \citep{MianNainer} give a method for designing equiripple minimum-phase FIR filters.  This method is based on that of Herrmann and Schuessler \citep{HerrmannSchuessler}, but avoids finding roots of polynomials, which posed a problem in the original method.  They accomplish this by using cepstral deconvolution with the FFT.  This method is useful in cases where linear-phase is not required or may be undesirable.  Instead, they design minimum-phase filters and reduce the filter length as well as the sensitivity of the coefficients to quantization errors.

The method of Herrmann and Shuessler \citep{HerrmannSchuessler} allows transformation of an equiripple linear-phase design into an equiripple minimum-phase design.  However, a difficulty with this method is that roots of high-order polynomials have to be taken to be factored suitably in order to obtain the minimum-phase design.  Mian and Nainer instead suggest an approach whereby the search for polynomial roots is avoided.  They show that by using a basic property of the complex cepstrum, the factorization problem can be solved simply by computing two FFT's, some complex logarithms and some other relatively simple operations.  It is known that numerical deconvolution can pose certain difficulties but the authors state that through experience, cepstral deconvolution works well and accurately in this particular case.

\subsection{The Performance of an Algorithm for Minimax Design of Two-Dimensional Linear Phase FIR Digital Filters -- Charalambous}

In his paper, Charalambous \citep{Charalambous} studies the problem of designing linear phase FIR filters in two dimensions using the minimax error criterion.  He uses one of his previous algorithms for minimax optimization and modifies the original problem into a sequence of weighted least squares problems.  The least squares functions are then minimized using the conjugate unconstrained algorithm from Powell.  Charalambous states that his method converges to the optimal solution and that there are no degeneracy problems.

The algorithm from Powell was chosen to be used in Charalambous'
method because of some of its advantages.  It needs only a few
operations to get its direction of search and also looks at any
symmetry that may be found in the optimization problem.  Therefore,
the algorithm does not need to search the whole space to get the
optimal solution.  This is a very useful property to have when the
problem becomes larger.

\subsection{Design of Almost Minimax FIR Filters in One and Two Dimensions by WLS Techniques -- Algazi et al.}

Algazi et al. \citep{Algazi} present a method for designing one- and two-dimensional FIR filters using weighted least squares techniques rather than the usually-preferred minimax method.  They state that the minimax method can be computationally intensive, particularly when dealing with two-dimensional problems.  They suggest the use of iterative WLS methods, even in the one-dimensional case.  These methods are then generalized for use in two dimensions.

The authors note that there is a relation between WLS and Chebyshev approximations and use this result for designing minimax filters using the WLS approach.  In one dimension, it is shown that the result is exactly the same for both methods.  They then extend it to two dimensions, obtaining an efficient and simple design technique.

WLS design consists of finding an optimal filter where the weighted least squares are minimized.  On the other hand, minimax design consists in minimizing the error in the Chebyshev sense by choosing proper filter coefficients.  Both techniques are iterative.  The Remez algorithm, which is used for minimax design, cannot be extended to two dimensions, however, since it depends on the alternation theorem which does not apply to two dimensions.  Instead, iterative ascent algorithms have been used but have been deemed computationally slow.

Algazi et al. recall the Lawson algorithm, which was used to find Chebyshev approximations by finding limits of sequences of weighted $L_p$ approximations.  The authors note that choosing $p=2$ gives a link between the WLS and Chebyshev approximations.  Lawson's algorithm can be applied as is to the one-dimensional problem and it will always converge, usually rather quickly.  However, there is a difficulty with Lawson's algorithm when some values unintentionally vanish after an iteration.  In this case, the solution is not optimal on the whole space but rather on a subset of the space.  

This method can also be used for designing FIR filters in two dimensions.  However, there is no proof that the result is actually a minimax FIR filter.  The lack of proof is related to the impossibility for the Remez algorithm to be extended to two dimensions.  Lawson's algorithm is quite simple to implement and the results obtained in one dimension are optimal therefore it can be a good alternative to other techniques which are more computationally complex.  The authors also note that in two dimensions, Chebyshev approximations are minimax but not equiripple since all the local extrema of the error do not typically reach the same maximum or minimum value.  

Now that they described an iterative method for designing FIR filters using WLS techniques, they then modify the algorithm in order to make the weights depend on the error from the previous iteration.  They change the weights at each iteration instead of waiting for the algorithm to converge before changing the weights according to Lawson's method.  However, they remind the readers that this method still does not guarantee that the result will be a minimax approximation.

\subsection{Design of FIR Filters in the Complex Domain -- Chen and Parks}

In this article, Chen and Parks \citep{ChenParks} take a look at the design of FIR digital filters using the Chebyshev error criterion, and where the frequency response is complex-valued.  They basically transform the complex problem into a real problem, then use linear programming to solve it.  They also add some more constraints which allow the phase and group delay to be weighted.  The idea is that they want to design filters which do not have exactly linear phase.  They mention that minimum phase FIR filters can introduce delay distortion if the delay is not constant over all frequencies.  For this reason, they determine that they approximation problem to be solved must be complex.  In order to solve this problem, they use the method of Glashoff and Roleff \citep{GlashoffRoleff} and Streit and Nuttall \citep{StreitNuttall} and apply it to the design of FIR filters before extending it to the design of FIR filters whose error in the pass-band group delay is small.

They remark that the linear complex problem can be seen as a nonlinear real optimization problem.  Further, they introduce a simple transformation which converts this nonlinear problem into a linear optimization problem.  They end up with a semi-infinite program, or Haar program, where there is a finite number of variables with an infinite number of conditions.  The authors mention two methods for solving this type of problem.  The first one applies an algorithm by Fahlander which is designed principally for this type of problem.  The second method consists of using a modified simplex method.  This involves finding the minimax solution of an overdetermined system of linear equations.  They consider this last approach and give a design procedure to be followed.  The first step is to change the original problem from the complex domain to the real domain, thus getting an overdetermined system of linear equations.  The second step consists of using linear programming to find a solution optimal in the Chebyshev sense.  In order to solve this problem, the authors use an algorithm which applies a modified simplex method to the dual problem.  This particular method does not need an initial estimate and always converges.  They also note that their results have nearly equiripple errors for the magnitude, the phase and the group delay.

\subsection{On the Design of Optimal Equiripple FIR Digital Filters for Data Transmission Applications -- Samueli}

Samueli \citep{Samueli} presents an improved algorithm based on linear programming, which is to be used to design equiripple FIR Nyquist filters as well as equiripple FIR transmit and receive matched filters.  Nyquist filters are defined as having an impulse response with uniformly spaced zero-crossings.  The transmit and receive matched filters can be used for data transmission and are actually a Nyquist filter when they are cascaded, therefore this method also applies to them.  The basic method consists of a linear programming section to compute a Nyquist filter whose frequency response is nonnegative, then a section where spectral factorization is used to obtain the nonlinear phase transmit and receive filters.

The transmit and receive filters used in data communication systems have constraints in the time domain.  Linear programming is typically the method of choice when dealing with such constraints.  However, there is usually a need for the frequency points to form a dense grid, which can lead to numerical ill-conditioning problems.  Samueli proposes a modification to the linear programming method whereby he avoids this necessity for a dense grid.  He states that technically, the linear program could be solved with only one inequality constraint per extremal frequency of the stop-band response.  However, the location of these frequencies is not known beforehand.  The author suggests that an iterative method be used to find these locations and thus reduce the amount of constraints.  After each iteration, the frequency grid points are chosen so that they are located at the extrema of the stop-band response.  He notes that this is similar to the Remez exchange algorithm.  In order to find these extrema, he uses Newton's method and searches for the zeros of the derivative of the frequency response.  These are then used as the grid points for the next iteration.  The extremal frequencies are then used to get the constraints on the maximum and minimum stop-band responses, alternatively evaluated.  The algorithm stops when the change in extrema is small enough.  The author cannot guarantee that this algorithm will always converge but his many numerical examples lead him to think it is very reliable.

The next step consists of taking the spectral factorization of the polynomial obtained at the previous step.  There are many methods which can be used for this step, including brute-force polynomial root-finding techniques.  Some tricks to reduce the computational complexity of this step are also given.  In the case of minimum and maximum phase transmit and receive matched filters, the author suggests using cepstral deconvolution in order to avoid polynomial root-finding.  This can be implemented using the FFT.

\subsection{On the Design of FIR Filters by Complex Chebyshev Approximation -- Preuss}

Preuss \citep{Preuss} considers the problem of designing an FIR filter to approximate a complex-valued function.  This algorithm solves the complex problem directly, without first transforming it into a real problem.  The author minimizes the magnitude of the complex error in the Chebyshev sense and uses a generalization of the Remez algorithm in order to do so.  

The problem here is to approximate a complex-valued frequency response.  The error function is complex and incorporates the weighted approximation error of both the magnitude and the phase at the same time.  The solution is the set of coefficients which minimize this error in the Chebyshev sense.  The minimized Chebyshev norm has an equiripple behaviour.  However, in this case, the error function which is comprised of both the magnitude error and the phase error is minimized.  Therefore, the magnitude error and the phase error by themselves do not end up having an equiripple behaviour, but are rather nearly equiripple.

Since there is no true equiripple behaviour, the Remez algorithm cannot be used here.  However, it can be generalized to be applicable to the complex problem.  This generalization can be simplified to the following four steps.  The first step is to compute all the extremal values of the error function as well as the frequencies corresponding to them.  The second step consists of choosing $n+1$ points out of the previous ones to be used for the next iteration.  The third step is to calculate the complex deviations at these points.  These are then used as the basis for the fourth step, which is the design of an interpolating transfer function using the previously-calculated points.  Usually, the extremal points and the angles of the error function change from one iteration to the next, and the differences become smaller.

In the case of linear phase filters, this method would ignore the symmetry of the coefficients but would still end up giving the same solution as with the Remez algorithm.  However, since the symmetry property is not used, it would be more time-consuming than simply using the Remez algorithm.  

\subsection{Improvements of a Complex FIR Filter Design Algorithm -- Schulist}

In this paper, Schulist \citep{Schulist} decided to take a look at the previously-presented Preuss algorithm \citep{Preuss} and improved upon it by accelerating its convergence.  The author also modifies the way the interpolated transfer function is computed, using a Gaussian relaxation algorithm rather than the Newton interpolation formula used by Preuss.

Schulist describes Preuss' algorithm, stating its many advantages, but not being satisfied with its convergence.  Preuss keeps the angles as entries for the interpolation part of his algorithm and this is what makes it in a way a generalization of the Remez algorithm.  However, the chosen magnitudes are what affect the convergence, and this is what the author wishes to work on.

The first improvement is in the calculation of the magnitudes of the error function.  Instead of prescribing these values, he writes a set of linear equations where the unknowns are the coefficients of the transfer function as well as the error magnitude.  He then solves for the error magnitude only, using Cramer's rule.  This gives a complex number, and its magnitude is then taken.  In the case where the error function has more extremal points than required, the author solves the overdetermined system of linear equations by using a Gaussian relaxation method.  Again, he only solves for the error magnitude.  

\sloppy
The second improvement concerns finding the impulse response by interpolation.  Preuss used Newton's formula with a chosen set of points which had the largest deviations.  Schulist decides to use all the extremal points and uses a Gaussian relaxation algorithm again to solve the overdetermined system of linear equations.  He then obtains a polynomial where the deviations are minimized in the mean squared sense.  In the case of nonlinear filters, this method worked very well.  However, it sometimes failed for nearly or exactly linear-phase filters.  In this case, the author recommends using the Newton interpolation formula instead. 

\fussy

\subsection{A Weighted Least Squares Algorithm for Quasi-Equiripple FIR and IIR Digital Filter Design -- Lim et al.}

Lim et al.\ \citep{Lim} present a new iterative algorithm for the design of FIR filters using a least squares frequency response weighting function.  The results have quasi-equiripple behaviour.

They compare the weighted least squares method to the Remez exchange algorithm and linear programming, stating that the former is well known and is easy to implement.  Another advantage of the WLS method over the others is that the optimal solution can be obtained analytically.  Observations have shown that WLS designs tend to also be optimal in the minimax sense, though a formal proof of this has not been done.  Basically, whether the WLS design is also optimal in the minimax sense depends on the way in which the necessary weighting function is obtained.  A new method for obtaining this weighting function is presented by the authors, who also state that the results will have an equiripple behaviour.

\sloppy
Frequency responses of linear phase FIR filters can be approximated as a sum of trigonometric functions multiplied by coefficients.  The error between the approximation and the desired functions can be found on a dense grid of frequencies and a set of linear equations can be formed from there.  The weighted least squares technique consists of solving a vector equation for the error and minimizing it.  The optimal solution can be found analytically but this is not the case for finding the least squares weighting function needed to get a solution which is optimal in the minimax sense.  Therefore, iterative methods are used.  

\fussy

The new algorithm proposed by Lim et al. is based on Lawson's algorithm and introduces an envelope function of the error function.  This envelope function is used instead of the error function itself in order to avoid some of the problems that Lawson's algorithm encounters when certain values vanish.  The envelope function will never be zero.  There is also a parameter in the function which can be modified to improve the convergence speed.  

The initial function needed to start the iteration can be set equal to the envelope function of the filter.  This can be obtained by rectangular windowing of the Fourier series of the ideal frequency response.  The parameter which can be modified and affects the convergence speed can be set by trial and error.  There is no analytical method for determining the value that will make the algorithm converge the fastest.  The authors state that their algorithm has about the same complexity as Lawson's algorithm.

The algorithm can terminate when one of several conditions are met.  One can set the number of iterations to be completed or quasi-equiripple behaviour can be checked as well.  This algorithm can be used in the design of FIR filters where the phase and the magnitude are arbitrarily prescribed.

\subsection{Optimal Design of FIR Filters with the Complex Chebyshev Error Criteria -- Burnside and Parks}

In their article, Burnside and Parks \citep{BurnsideParks} describe an algorithm which is a variation on the simplex algorithm.  It can be used to design FIR filters that approximate complex-valued frequency responses.  This method has also been used to design filters of length $1000$.

The complex approximation problem can be seen as a nonlinear real approximation problem, and can even be reformulated as a linear approximation problem.  In this case, an exact parametrization is used, and there is no need to worry about approximation errors.  The linear program related to this problem is a continuous, semi-infinite program.  It has an uncountable set of constraint parameters.  This linear program can be reformulated as a dual linear program, which is related to the primal problem.  The authors state some advantages to using the dual formulation rather than the primal formulation.  First, the dimension of the constraints is reduced.  It is also known that this type of problem has a strong duality property.  Therefore, once one solution is found, the other one is very easy to find as well.  Another advantage is that the dual variables are Lagrange multipliers of the active constraints at the solution point.  Using this property lets one analyze the sensitivity of the solution very easily.

The new algorithm is as follows.  The first step is to find a basic feasible solution.  The authors compare three methods for choosing the starting point: the conventional artificial variable method, a method by Cuthbert, and a method by Tang.  The latter is too ill-conditioned for their use, and Cuthbert's method does not let them add more linear constraints, therefore, they settle on the artificial variable method.  In the second step, they calculate the primal and dual variables.  Then, the third step consists of pricing a fine grid of constraints.  This step is different than in the standard simplex algorithm.  They use a partial pricing algorithm for this step.  This algorithm first solves the linear program for choosing the best pricing for the variables, calculating the error function related to the solution and, if the algorithm has not converged yet, restarting another iteration with values redefined to take into account the local maxima of the weighted error function.  This is basically a multiple exchange method because each block iteration ends up exchanging all the local extrema of the error function.  At each iteration, the linear program uses the previous solution as its basis.  The authors, through experimentation, found that it is better to keep all the additional constraints instead of dropping those that are inactive when new ones are added.  After the partial pricing, the nonbasic gradient pivoting rule is used to select the columns of the matrix to be entered into the basis.  The fourth step consists of generating a column corresponding to the incoming variable.  The fifth step is simply a ratio test.  The authors used an anti-cycling method proposed by Steiglitz, which seems to work well for this method.

This algorithm can be used to design both real- and complex-valued coefficient filters.



==> abstract.tex <==
Image resampling is a necessary component of any operation that
changes the size of an image or its geometry.

Methods tuned for natural image upsampling (roughly speaking, image
enlargement) are analyzed and developed with a focus on their ability
to preserve diagonal features and suppress overshoots. Monotone,
locally bounded and almost monotone ``direct'' interpolation and
filtering methods, as well as face split and vertex split surface
subdivision methods, alone or in combination, are studied. Key
properties are established by way of proofs and counterexamples as
well as numerical experiments involving 1D curve and 2D diagonal data
resampling.

In addition, the Remez minimax method for the computation of low-cost
polynomial approximations of low-pass filter kernels tuned for natural
image downsampling (roughly speaking, image reduction) is refactored
for relative error minimization in the presence of roots in the
interior of the interval of approximation and so that even and odd
functions are approximated with like polynomials. The accuracy and
frequency response of the approximations are tabulated and plotted
against the original, establishing their rapid convergence.


==> acknowledgements.tex <==
There are many people who have helped make this thesis possible and to
whom I am deeply grateful.  I would first like to thank my thesis
supervisor, Dr.~Nicolas Robidoux, for his countless hours of work, his
dedication and his patience.  He was always available to answer any
question and gave me much good advice.  His energy, enthusiasm and
commitment motivated me to continue working while his honesty and
selfless support has made him the best supervisor I could have hoped
for.

I am grateful to my co-supervisor, Dr.~Julien Dompierre, for always
believing in me and offering me his support and his help.  I also
thank Dr.~Ralf Meyer for all his help through the completion of this
degree, from writing me a letter of recommendation to helping with the
choice of courses.  His help has made this experience a lot smoother.
I am thankful to Dr.~Richard Bartels for taking the time to read this paper and for offering useful advice and comments.

I also extend my gratitude to Dr.~Fabrice Colin for taking the time to advise me on how to approach certain mathematical problems.

I wish to thank Louise Rancourt, Aaron Langille, Mark Thompson and Linda Weber for everything they did, from setting up a computer and desk for my use to keeping the department running smoothly and helping me with the registration procedure.  I am also grateful to Dr.~Kalpdrum Passi for his guidance and his help throughout my studies.  His devotion to the students make him an ideal department chair and made him a great graduate coordinator.


==> dedication.tex <==
To my family and friends, for being there for me.



==> dummy.tex <==
 

==> funding.tex <==
The author of this thesis was supported by an NSERC (National Science
and Engineering Research Council) Alexander Graham Bell Canada
Graduate Scholarship, by an NSERC Discovery Grant awarded to
Dr.~J.~Dompierre, by a grant from the NIGMS (National Institute of
General Medical Sciences) Center for the Spatiotemporal Modeling of
Cell Signaling at the University of New Mexico awarded to
Dr.~N.~Robidoux, and by Laurentian University through a GTA (Graduate
Teaching Assistantship) and Dr.~Robidoux's professional allowance.

